Rational subsets of Baumslag-Solitar groups

We consider the rational subset membership problem for Baumslag-Solitar groups. These groups form a prominent class in the area of algorithmic group theory, and they were recently identified as an obstacle for understanding the rational subsets of $\text{GL}(2,\mathbb{Q})$. We show that rational subset membership for Baumslag-Solitar groups $\text{BS}(1,q)$ with $q\ge 2$ is decidable and PSPACE-complete. To this end, we introduce a word representation of the elements of $\text{BS}(1,q)$: their pointed expansion (PE), an annotated $q$-ary expansion. Seeing subsets of $\text{BS}(1,q)$ as word languages, this leads to a natural notion of PE-regular subsets of $\text{BS}(1, q)$: these are the subsets of $\text{BS}(1,q)$ whose sets of PE are regular languages. Our proof shows that every rational subset of $\text{BS}(1,q)$ is PE-regular. Since the class of PE-regular subsets of $\text{BS}(1,q)$ is well-equipped with closure properties, we obtain further applications of these results. Our results imply that (i) emptiness of Boolean combinations of rational subsets is decidable, (ii) membership to each fixed rational subset of $\text{BS}(1,q)$ is decidable in logarithmic space, and (iii) it is decidable whether a given rational subset is recognizable. In particular, it is decidable whether a given finitely generated subgroup of $\text{BS}(1,q)$ has finite index.

==> iteration.tex <==

Some natural strategies to prove \Cref{main-effective-regularity}
face the following obstacle:
PE-regular sets as per our \Cref{def:regular}
are not closed under iteration (Kleene star).

\begin{example}
Consider the PE-regular set
$A = \{ v \in \BS(1,2) \mid \pe(v) \in + \cursor{\rpoint{1}} 0^* 1 \}$,
which contains exactly all elements $a t^{-n} a t^n$, $n \ge 1$.
The iteration
$A^* = \{ g_1 \cdot \ldots \cdot g_k \mid \text{each $g_i \in A$; $k \ge 0$} \}$
is a set of the form $W \times \{ 0 \}$, because
each $g_i$ returns the cursor to the origin
(if we think of an automaton over the infinite tape with binary alphabet,
 then for such a return it would need to ``sense'' the radix point).
Here $W = \{ v_1 + \ldots + v_k \mid
             \text{each $v_i = 1 + 2^{-d_i}$ for some $d_i \ge 1$; $k \ge 0$} \}$.

We show that $W \times \{ 0 \}$ is not PE-regular.
Indeed, suppose it were. Consider another PE-regular set,
$R = \{ v \in \BS(1,2) \mid
        \pe(v) \in + \{0,1\}^* \{\cursor{\rpoint{0}}, \cursor{\rpoint{1}}\} 1^* \}$.
The intersection $(W \times \{0\}) \cap R$ should then be a PE-regular set
by \Cref{main-closure-properties}.
For each $n \ge 1$, consider the following set, which is the restriction
of a right quotient of $(W \times \{0\}) \cap R$ to (expansions of) integers:
\begin{equation*}
Y = \{ w \in \Phi_2^* \mid
       \text{there is $v \in (W \times \{0\}) \cap R$ such that
             $\pe(v) = w \cdot 1^n$} \}
    \cap
    \{ 0, 1 \}^* \{ \cursor{\rpoint{0}}, \cursor{\rpoint{1}} \}
\enspace.
\end{equation*}
Note that the $n$ binary $1$s in the right factor of $\pe(v)$ occur
after the radix point, and whenever $v = v_1 + \ldots + v_k$, $v_i = 1 + 2^{-d_i}$,
each $v_i$ can contribute at most one~$1$.
So $k \ge n$; therefore, $v \ge n$ and the smallest number with a pointed expansion
in $Y$ is~$n$.
But since $Y$ is regular (due to standard closure properties of regular languages),
this means that $(W \times \{0\}) \cap R$ has infinitely many right quotients
(one for each $1^n$),
which contradicts the Myhill--Nerode theorem.
\end{example}

